On the functoriality of Khovanov homology

We provide an overview of Blanchet's oriented model of Khovanov homology, which resolves the sign ambiguity in functoriality. We give a detailed and self-contained exposition of the construction. We establish strict functoriality for the oriented model and briefly outline its extension to cobordisms with singularities recently studied by Scott Carter, Benjamin Cooper, Mikhail Khovanov and Vyacheslav Krushkal.

==> Text/MM18.tex <==
\textbf{MM18:}

==> Text/MMTwelve.tex <==
\textbf{MM12+:} 
The left side of $MM12 $ is a cap followed by $R_1+$.\\
\[\begin{tikzcd}[row sep=1.5cm, column sep=1cm]
0 \arrow[r]& \emptyset 
\arrow[d]
\arrow[d,phantom,dash,"{\inlinepic{
    \begin{scope}[scale=0.3]
    \BCapE{}{+}
    \end{scope}
    }}"xshift=1cm]
\arrow[r]& 0\\ 
0 \arrow[r]& 
\inlinepic{
    \begin{scope}[scale=0.4]
        \Circle{-}
    \end{scope}
}
\arrow[d]
\arrow[d,phantom,dash,"{
    \inlinepic{
    \begin{scope}[scale=0.2]
        \BRCapE{1}{-}{}{}
        \begin{scope}[xshift=3cm,yshift=2cm]
            \BCylE{}{-}{-}
        \end{scope}
    \end{scope}
    }\quad - \quad
    \inlinepic{
    \begin{scope}[scale=0.2]
        \BRCapE{}{-}{}{}
        \begin{scope}[xshift=3cm,yshift=2cm]
            \BCylE{1}{-}{-}
        \end{scope}
    \end{scope}
    }
}"xshift=2cm]
\arrow[r]& 0\\ 
0 \arrow[r] & 
\inlinepic{
    \begin{scope}[scale=0.4]
        \Circle{+}
        \begin{scope}[xshift=2cm]
            \Circle{-}
        \end{scope}
    \end{scope}
} \arrow[r]& 
\inlinepic{
    \begin{scope}[scale=0.15]
             \begin{scope}
                \clip (0,3) rectangle (4.5,-3);
                \draw[draw=Blue,postaction={decorate}, decoration={markings, mark=at position 0.25 with {\arrow{<}}}] (1.5,0) circle (2cm);
            \end{scope}

            \begin{scope}
                \clip (0,3) rectangle (-4.5,-3);
                \draw[draw=Blue,postaction={decorate}, decoration={markings, mark=at position 0.25 with {\arrow{>}}}] (-1.5,0) circle (2cm);
            \end{scope}
            \begin{scope}
                \clip  (1.5,0) circle (2cm);
                \draw[draw=Maroon,thick,postaction={decorate}, decoration={markings, mark=at position 0.7 with {\arrow[scale=0.7]{>>}}}] (0,-2)--(0,2);
            \end{scope}
    \end{scope}
}\arrow[r]\vspace{0.5cm}&0
\end{tikzcd}
\]
The resulting map $f$ going from $\emptyset$ to 
\inlinepic{
    \begin{scope}[scale=0.3]
        \Circle{+}
        \begin{scope}[xshift=2cm,]
            \Circle{-}
        \end{scope}
    \end{scope}
} is $f=$ \quad 
    \inlinepic{
    \begin{scope}[scale=0.3]
        \BRCapE{1}{-}{}{}
        \begin{scope}[xshift=3cm]
            \BCapE{}{-}
        \end{scope}
    \end{scope}
    }\quad - \quad
    \inlinepic{
    \begin{scope}[scale=0.3]
        \BRCapE{}{-}{}{}
        \begin{scope}[xshift=3cm]
            \BCapE{1}{-}
        \end{scope}
    \end{scope}
    }.
    \vspace{0.5cm}\\
    %
    %
    %
    The right side of MM12 is a cup followed by $R_1'+$. 
\[\begin{tikzcd}[row sep=2cm, column sep=1cm]
0 \arrow[r]& \emptyset 
\arrow[d]
\arrow[d,phantom,dash,"{\inlinepic{
    \begin{scope}[scale=0.4]
    \BCapE{}{-}
    \end{scope}
    }}"xshift=1cm]
\arrow[r]& 0\\ 
0 \arrow[r]& 
\inlinepic{
    \begin{scope}[scale=0.5]
        \Circle{+}
    \end{scope}
}
\arrow[d]
\arrow[d,phantom,dash,"{
    \inlinepic{
    \begin{scope}[scale=0.3]
        \BRCapE{1}{+}{}{}
        \begin{scope}[xshift=-3cm,yshift=2cm]
            \BCylE{}{+}{+}
        \end{scope}
    \end{scope}
    }\quad - \quad
    \inlinepic{
    \begin{scope}[scale=0.3]
        \BRCapE{}{+}{}{}
        \begin{scope}[xshift=-3cm,yshift=2cm]
            \BCylE{1}{+}{+}
        \end{scope}
    \end{scope}
    }
}"xshift=3cm]
\arrow[r]& 0\\ 
0 \arrow[r] & 
\inlinepic{
    \begin{scope}[scale=0.5]
        \Circle{+}
        \begin{scope}[xshift=2cm]
            \Circle{-}
        \end{scope}
    \end{scope}
} \arrow[r]& 
\inlinepic{
    \begin{scope}[scale=0.2]
             \begin{scope}
                \clip (0,3) rectangle (4.5,-3);
                \draw[draw=Blue,postaction={decorate}, decoration={markings, mark=at position 0.25 with {\arrow{>}}}] (1.5,0) circle (2cm);
            \end{scope}

            \begin{scope}
                \clip (0,3) rectangle (-4.5,-3);
                \draw[draw=Blue,postaction={decorate}, decoration={markings, mark=at position 0.25 with {\arrow{<}}}] (-1.5,0) circle (2cm);
            \end{scope}
            \begin{scope}
                \clip  (1.5,0) circle (2cm);
                \draw[draw=Maroon,thick,postaction={decorate}, decoration={markings, mark=at position 0.7 with {\arrow[scale=0.7]{<<}}}] (0,-2)--(0,2);
            \end{scope}
    \end{scope}
}\arrow[r]\vspace{0.5cm}&0
\end{tikzcd}
\]
The resulting map $f$ going from $\emptyset$ to 
\inlinepic{
    \begin{scope}[scale=0.3]
        \Circle{+}
        \begin{scope}[xshift=2cm,]
            \Circle{-}
        \end{scope}
    \end{scope}
} is $f=$ \quad 
    \inlinepic{
    \begin{scope}[scale=0.3]
        \BRCapE{1}{-}{}{}
        \begin{scope}[xshift=3cm]
            \BCapE{}{-}
        \end{scope}
    \end{scope}
    }\quad - \quad
    \inlinepic{
    \begin{scope}[scale=0.3]
        \BRCapE{}{-}{}{}
        \begin{scope}[xshift=3cm]
            \BCapE{1}{-}
        \end{scope}
    \end{scope}
    }.
    \vspace{0.5cm}\\


==> Text/SInvariant.tex <==
\section{The $s$-invariant}
\subsection{Some terminology} 
Let $(C,d)$ be a chain complex. A finite length filtration on $C$ is a sequence of subcomplexes $\{F^iC\}_{i}$    such that: 
\[0=F^nC\subseteq F^{n-1}C\subseteq ... \subseteq F^{m-1}C\subseteq F^mC=C\]
We associate a grading to the filtration by setting $deg(x)=i$ if $x\in F^iC\setminus F^{i+1}C$. 
If $f$ is a map between two filtered complexes $(C_1,d_1)$ and $(C_2,d_2)$, we say that $f$ is a filtered map if $f(F^iC_1)\subseteq F^iC_2$ for all $i$. If $f$ is a filtered map, we define its degree by $deg(f)=k$ if $f(F^iC_1)\subseteq F^{i+k}C_2$ for all $i$.\\
A filtration on $C$ induces a filtration $s$ on its homology $H(C)$ by setting $F^iH(C)=Im(H(F^iC)\rightarrow H(C))$.\\ If $f$ is a filtered map between two filtered complexes, it induces a map $H(f):H(C_1)\rightarrow H(C_2)$ between their homologies, which is also a filtered map of the same degree as $f$.\\
A finite length filtration on a complex $(C,d)$ induces a spectral sequence, which converges to the associated graded object of the homology $H(C)$ of $C$. 
 
\subsection{The definition of the $s$-invariant}
Let $K$ be a knot. 
In section \ref{sec:RecoveringKh}, we showed that there exists a basis in which $\mathcal{T}(CKh(K))\sim Kh(K)$ has differentials $m$ (for merging two circles) and $\Delta$ (for splitting a circle) defined by:\\
\[\begin{array}{l l}
    m(1\otimes 1)=1 \hspace{2cm}& \Delta(1)=1\\
    m(1\otimes X)=X \hspace{2cm}& \Delta(X)=X\otimes X\\
    m(X\otimes 1)=X \hspace{2cm}& \\    
    m(X\otimes X)=0 &
\end{array}\]
Similarly, we can prove that the Lee Khovanov homology $CKh'(K)$ is isomorphic to a complex that has differentials $m'$ and $\Delta'$ given by:\\
\[\begin{array}{l l}
    m'(1\otimes 1)=1 \hspace{2cm}& \Delta'(1)=1\otimes X+X\otimes 1\\
    m'(1\otimes X)=X \hspace{2cm}& \Delta'(X)=1\otimes 1+X\otimes X\\
    m'(X\otimes 1)=X \hspace{2cm}& \\    
    m'(X\otimes X)=1    &
\end{array}\]

The complex $Kh$ is graded, with $\deg(1)=1$ and $\deg(X)=-1$. In contrast, $CKh'$ is not graded but it has a filtration induced by the grading on $CKh$. In fact, $m'-m$ and $\Delta'-\Delta$ both have degree $4$. 
\begin{thh}
    There is a spectral sequence with $E_1$ page $CKh'(L)$, $E_2$ page $H(Kh(L)\otimes \mathbb{Q})$ and converging to $\mathcal{L}Kh(L)$ the homology of the complex $CKh'(L)$.\\
    This spectral sequence is an invariant of the link $L$.
\end{thh}
\begin{proof}
    The first statement follows from the observation above that $m'-m$ and $\Delta'-\Delta$ have degree $4$.
    \\ The second statement is a result of lemma \ref{invarianceOfFiltered}.
\end{proof}
\begin{lemma}
\label{invarianceOfFiltered}
    Let $F:C_1\rightarrow C_2$ be a filtered chain map between two filtered complexes $(C_1,d_1)$ and $(C_2,d_2)$. Then induces a map of spectral sequences $E_i(F):E_i(C_1)\rightarrow E_i(C_2)$ for all $i\geq 1$. If $F_n$ is an isomorphism for a certain $n\geq 1$, then $F_i$ is an isomorphism for all $i\geq n$.
\end{lemma}
A proof of this lemma can be found in \cite{Rasmussen2010}.\par
Theorem \ref{LeeDegeneration} states that the homology $\mathcal{L}Kh(K)$ of $CKh'(K)$ is $\mathbb{Q}\oplus \mathbb{Q}$ for a knot $K$. The two generators are in odd homological degree. Let $s_{min}(K)$ and $s_{max}(K)$ be the filtration degrees of these two generators, such that $s_{max}(K)\geq s_{min}(K)$. $s_{min}$ and $s_{max}$ are invariants of the knot $K$, since the homotopy equivalences defined in the proof of theorem \ref{invariance} are filtered maps of degree $0$. \\
\begin{prop}
    \label{sinvariant}
    For any knot $K$, $s_{max}(K)=s_{min}(K)+2$. 
\end{prop}
Rasmussen uses this proposition to define the $s$-invariant of a knot $K$ by $s(K)=s_{max}(K)-1=s_{min}(K)+1$.\\
\subsection{Proof of proposition \ref{sinvariant}}
A few preliminary lemmas are needed. 
\begin{lemma}
    \label{decomposition}
    Let $K$ be a knot. There is a direct sum decomposition $CKh'(K)=CKh'_0(K)\oplus CKh'_1(K)$, where $CKh'_0(K)$ is the subspace of $CKh'(K)$ generated by elements in homological degree $3$ mod $4$ and $CKh_1(K)$ is the subspace generated by elements in homological degree $1$ mod $4$. \\
    Let $s_a$ be the oriented resolution of $K$ with labels $a$ on all circles, and $s_b$ be the oriented resolution with labels $b$ on all circles. Then $(s_a+s_b)$ is contained in one of these subcomplexes, and $(s_a-s_b)$ is contained in the other.
\end{lemma}
\begin{cor}
    $s(s_a)=s(s_b)=s_{min}(K).$
\end{cor}
\begin{cor}
    \label{corollary}
    $s_{max}(K)>s_{min}(K).$
\end{cor}
The proof of lemma \ref{decomposition} as well as corollary \ref{corollary} are the same as in section 3 of \cite{Rasmussen2010}.\\
\begin{lemma}
    For two knots $K_1$ and $K_2$, there is a short exact sequence
    \[
    \begin{tikzcd}
    0 \arrow[r] &  CKh'(K_1 \# K_2) \arrow[r,"p_*"] & CKh'(K_1)\otimes CKh'(K_2) \arrow[r,"\partial"] & CKh'(K_1\inlinepic{
                \begin{scope}[scale=0.8]
                    \draw[Blue,->] (0,0.2) to[in=-120,out=0] (60:0.4);
                    \draw[Blue,->] (0,0.2) to[in=-60,out=180] (120:0.4);
                    \draw[Maroon,thick,decoration={ markings, mark=at position 0.7 with {\arrow[scale=0.5]{>>}}},postaction={decorate}] (0,-0.2)--(0,0.2);
                    \draw[Blue] (-60:0.4) to[in=0, out=120] (0,-0.2);
                    \draw[Blue] (-120:0.4) to[in=180, out=60] (0,-0.2);
                \end{scope}
            }K_2) \arrow[r] & 0
    \end{tikzcd}\]
    Where $p^*$ and $\partial$ are filtered maps of degree $-1$.
\end{lemma}
\textcolor{red}{Proof of this lemma}
\begin{proof}of proposition \ref{sinvariant}\par
    Consider the short exact sequence above for $K_1=K$ and $K_2=$\inlinepic{\begin{scope}[scale=0.25]\Circle{-}
    \end{scope}
        }. 
    Let $s_a$ be the oriented resolution of $K$ with labels $a$ on all circles, and $s_b$ be the oriented resolution with labels $b$ on all circles. We can assume that $s_a-s_b=s_{max}(K)$. Let $a=$ \inlinepic{\begin{scope}[scale=0.25]\Circle{-}
        \node at (1.2,0) {\tiny$a$};
    \end{scope}
        } and $b=$ \inlinepic{\begin{scope}[scale=0.25]\Circle{-}
        \node at (1.2,0) {\tiny$b$};
    \end{scope}
        }.  The map $\partial$ sends $(s_a-s_b)\otimes a$ to $s_a$\inlinepic{
                \begin{scope}[scale=0.8]
                    \draw[Blue,->] (0,0.2) to[in=-120,out=0] (60:0.4);
                    \draw[Blue,->] (0,0.2) to[in=-60,out=180] (120:0.4);
                    \draw[Maroon,thick,decoration={ markings, mark=at position 0.7 with {\arrow[scale=0.5]{>>}}},postaction={decorate}] (0,-0.2)--(0,0.2);
                    \draw[Blue] (-60:0.4) to[in=0, out=120] (0,-0.2);
                    \draw[Blue] (-120:0.4) to[in=180, out=60] (0,-0.2);
                \end{scope}
            }$a$. \\
    By the band relation there is a degree $0$ isomorphism sending $s_a$\inlinepic{
                \begin{scope}[scale=0.8]
                    \draw[Blue,->] (0,0.2) to[in=-120,out=0] (60:0.4);
                    \draw[Blue,->] (0,0.2) to[in=-60,out=180] (120:0.4);
                    \draw[Maroon,thick,decoration={ markings, mark=at position 0.7 with {\arrow[scale=0.5]{>>}}},postaction={decorate}] (0,-0.2)--(0,0.2);
                    \draw[Blue] (-60:0.4) to[in=0, out=120] (0,-0.2);
                    \draw[Blue] (-120:0.4) to[in=180, out=60] (0,-0.2);
                \end{scope}
            }$a$ to $s_a$. Therefore $s(s_a$\inlinepic{
                \begin{scope}[scale=0.8]
                    \draw[Blue,->] (0,0.2) to[in=-120,out=0] (60:0.4);
                    \draw[Blue,->] (0,0.2) to[in=-60,out=180] (120:0.4);
                    \draw[Maroon,thick,decoration={ markings, mark=at position 0.7 with {\arrow[scale=0.5]{>>}}},postaction={decorate}] (0,-0.2)--(0,0.2);
                    \draw[Blue] (-60:0.4) to[in=0, out=120] (0,-0.2);
                    \draw[Blue] (-120:0.4) to[in=180, out=60] (0,-0.2);
                \end{scope}
            }$a)=s(s_a)=s_{min}(K)$.
            \\
    $\partial$ is filtered of degree $-1$, Therefore $s((s_a-s_b)\otimes a)\leq s(s_a)+1$. But $s((s_a-s_b)\otimes a)=s_{max}(K) -1$ and $s(s_a)=s_{min}(K)$. So $s_{max}(K)-1\leq s_{min}(K)+1$. And $s_{max}(K)\leq s_{min}(K)+2$. 
\end{proof}
\subsection{The slice genus}
The main theorem of \cite{Rasmussen2010} is the following:
\begin{thh}
    \label{slicegenus}
    For any knot $K$, $|s(K)|\leq 2g_*(K)$, where $g_*(K)$ is the slice genus of $K$.
\end{thh}
\begin{proof}
    Let $K$ be a knot that bounds a surface $\Sigma$ of genus $g$ in the $4$-ball. Then there is an orienteable connected cobordism $\Sigma$ of Euler characteristic $-2g$ from $K$ to the unknot. By functoriality of Khovanov homology, this cobordism induces a filtered map $(CKh'(\Sigma)):CKh'(K)\rightarrow CKh'(\inlinepic{\draw (0,0)circle (0.2cm);})$ of degree $-2g$. \\
    So for any $x\in CKh'(K)$, $s((CKh'(\Sigma))(x))\geq s(x)-2g$.\\ 
    The slice genus of the unknot is $0$, $s_{max}(\inlinepic{\draw (0,0)circle (0.2cm);})=1$. So $1\geq s(x)-2g$ for all $x\in CKh'(K)$, and in particular for $x$ a generator of filtration degree $s_{max}(K)$. Therefore $1\geq s_{max}(K)-2g$, and $s(K)\leq 2g$.\\
    Using the same argument for the mirror image of $K$ \textcolor{red}{....}
\end{proof}
